Scaling Up Probabilistic Circuits by Latent Variable Distillation

Probabilistic Circuits (PCs) are a unified framework for tractable probabilistic models that support efficient computation of various probabilistic queries (e.g., marginal probabilities). One key challenge is to scale PCs to model large and high-dimensional real-world datasets: we observe that as the number of parameters in PCs increases, their performance immediately plateaus. This phenomenon suggests that the existing optimizers fail to exploit the full expressive power of large PCs. We propose to overcome such bottleneck by latent variable distillation: we leverage the less tractable but more expressive deep generative models to provide extra supervision over the latent variables of PCs. Specifically, we extract information from Transformer-based generative models to assign values to latent variables of PCs, providing guidance to PC optimizers. Experiments on both image and language modeling benchmarks (e.g., ImageNet and WikiText-2) show that latent variable distillation substantially boosts the performance of large PCs compared to their counterparts without latent variable distillation. In particular, on the image modeling benchmarks, PCs achieve competitive performance against some of the widely-used deep generative models, including variational autoencoders and flow-based models, opening up new avenues for tractable generative modeling. Our code can be found at https://github.com/UCLA-StarAI/LVD.

==> tikz/tikzlibrarypc.code.tex <==
% Copyright 2016 by Nicola Di Mauro and Antonio Vergari
%
% This file may be distributed and/or modified
%
% under the GNU General Public License.
%
% See the files LICENSE for more details.

\usetikzlibrary{chains}
%\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usepackage{xparse}
%\usepackage{listofitems}

%\newif\iflabelleft

\newdimen\mywidth
\newdimen\myheight

\newcommand*{\IfStringInList}[2]{%
  \in@{,#1,}{,#2,}%
  \ifin@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

% sum node style
\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

% product node style
\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

% \sumnode [tikz-options] {sum node name} 
\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

% \prodnode [tikz-options] {product node name} 
\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

% \maxnode [tikz-options] {max node name} 
\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

% \emptynode [tikz-options] {generic node name}
\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}


\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodeleft}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodedown}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {#3};
}

\newcommand{\cbernodedown}[4][]{
  \node[circle,fill=white,draw=#4,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw[draw=#4] circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {\textcolor{#4}{#3}};
}

\DeclareDocumentCommand{\contnode}{o m m o}  
{%
  \IfNoValueTF{#4}
  {\contnodebelow[#1]{#2}{#3}}
  {\contnodeleft[#1]{#2}{#3}}
}

\newcommand{\contnodebelow}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture}
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnodeleft}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} 
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnodedown}[4][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} 
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none,draw=#4] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[below=0pt of #2, xshift=0pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\cedge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[-,#1] (\x)+(0,-9pt) -- ($(0,9pt)+(\y)$);
      % \path ([yshift=9pt]\x) edge [-,#1] ([yshift=9pt]\y) ;%
    } ;
  } ;
}

\newcommand{\mycedge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[-,#1] (\x)+(0,-9pt) -- ($(-6.0pt,6.0pt)+(\y)$);
      % \path ([yshift=9pt]\x) edge [-,#1] ([yshift=9pt]\y) ;%
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}

\newcommand{\colorweigedge}[7][]{
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;
      % \draw[rounded corners] ($(\x)!0.5!(\y)$) rectangle node{#4} (\y) ;
      \pgfmathparse{width("\noexpand\noexpand\noexpand#4")} ; %the width calc
      \pgfmathsetlength{\mywidth}{\pgfmathresult} ; % Put it into a length register
      \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %the height calc
      \pgfmathsetlength{\myheight}{\pgfmathresult} ; % Put it into a length register
      \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#6,text=#7,minimum height=1.8\myheight,minimum width=1.2\mywidth,label={center:\textcolor{#7}{#4}}] at ($(\x)!0.5!(\y)$) {} ;
    } ;
  } ;
}

\newcommand{\ellipsis}[2]{
  \node at ($(#1)!.5!(#2)$) {\ldots} ;
}

\newcommand{\annotatenode}[4]{
  \node[] at ([xshift=#3,yshift=#4]#1) {#2} ;
}

\newcommand{\colorfulannotnode}[6]{
  \pgfmathparse{width("\noexpand\noexpand\noexpand#2")} ; %the width calc
  \pgfmathsetlength{\mywidth}{\pgfmathresult} ; % Put it into a length register
  \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %the height calc
  \pgfmathsetlength{\myheight}{\pgfmathresult} ;
  \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#5,text=#6,minimum height=1.3\myheight,minimum width=1.3\mywidth,label={center:\textcolor{#6}{#2}}] at ([xshift=#3,yshift=#4]#1) {} ;
}

\newcommand{\midlinewidth}{1.0pt}
\newcommand{\incmidlinewidth}{1.7pt}
\newcommand{\largelinewidth}{1.9pt}
\newcommand{\xlargelinewidth}{2.3pt}
\newcommand{\middist}{17pt}
\newcommand{\sqintermiddist}{15.5pt}
\newcommand{\intermiddist}{30pt}
\newcommand{\largedist}{49pt}
\newcommand{\midsmalldist}{10pt}
\newcommand{\smalldist}{6pt}
\newcommand{\tinydist}{4pt}
\newcommand{\centraldist}{30pt}
\newcommand{\midlargedist}{24pt}
\newcommand{\halfdist}{19pt}
\newcommand{\weightsize}{\fontsize{10}{10}\selectfont}
\newcommand{\annotsize}{\fontsize{10}{10}\selectfont}

\definecolor{lacamlilac} {RGB} {107,93,153}
\definecolor{lacamlilac2} {RGB} {93, 109, 152}
\definecolor{lacamlightlilac} {RGB} {174, 166, 201}
\definecolor{lacamdarklilac} {RGB} {51, 10, 102}
\definecolor{lacamdarklilac5} {RGB} {51, 10, 102}
\colorlet{lacamdarklilac4} {lacamdarklilac5!80!}
\colorlet{lacamdarklilac3} {lacamdarklilac5!60!}
\colorlet{lacamdarklilac2} {lacamdarklilac5!40!}
\colorlet{lacamdarklilac1} {lacamdarklilac5!20!}

\definecolor{lacamgold5} {RGB} {255, 87, 0}
\colorlet{lacamgold4} {lacamgold5!80!}
\colorlet{lacamgold3} {lacamgold5!60!}
\colorlet{lacamgold2} {lacamgold5!40!}
\colorlet{lacamgold1} {lacamgold5!20!}
\definecolor{violet} {RGB} {119, 111, 178}
\definecolor{petroil2} {RGB} {36, 165, 175}
\definecolor{petroil4} {RGB} {30, 132, 149}
\definecolor{petroil6} {RGB} {23, 101, 115}
\definecolor{gold2} {RGB} {255, 130, 0}
\definecolor{gold4} {RGB} {250, 100, 0}
\definecolor{gold6} {RGB} {245, 90, 0}

\definecolor{lacamoil5}{rgb}{0.13, 0.67, 0.8}
\colorlet{lacamoil4} {lacamoil5!80!}
\colorlet{lacamoil3} {lacamoil5!60!}
\colorlet{lacamoil2} {lacamoil5!40!}
\colorlet{lacamoil1} {lacamoil5!20!}

\definecolor{lightgray} {RGB} {210, 210, 210}
\definecolor{myblue} {RGB} {80, 145, 207}
\definecolor{mypurple} {RGB} {101, 43, 150}
\definecolor{myred} {RGB} {255, 0, 1}

\definecolor{mycolor1}{HTML}{781C68}
\definecolor{mycolor2}{HTML}{277BC0}
\definecolor{mycolor3}{HTML}{FFB200}

%\definecolor{tomato0} {HTML} {E57373}
\definecolor{tomato0} {HTML} {EF9A9A}
\definecolor{tomato1} {HTML} {F44336}
\definecolor{tomato2} {HTML} {E53935}
\definecolor{tomato3} {HTML} {D32F2F}
\definecolor{tomato4} {HTML} {C62828}
\definecolor{tomato5} {HTML} {B71C1C}


\definecolor{peas1} {HTML} {009688}
\definecolor{peas2} {HTML} {00897B}
\definecolor{peas3} {HTML} {00796B}
\definecolor{peas4} {HTML} {00695C}
\definecolor{peas5} {HTML} {004D40}

\definecolor{bgrey0} {HTML} {78909C}
\definecolor{bgrey1} {HTML} {607D8B}
\definecolor{bgrey2} {HTML} {546E7A}
\definecolor{bgrey3} {HTML} {455A64}
\definecolor{bgrey4} {HTML} {37474F}
\definecolor{bgrey5} {HTML} {263238}

\definecolor{olive0} {HTML} {C5E1A5}
\definecolor{olive1} {HTML} {AED581}
\definecolor{olive2} {HTML} {9CCC65}
\definecolor{olive3} {HTML} {8BC34A}
\definecolor{olive4} {HTML} {7CB342}
\definecolor{olive5} {HTML} {689F38}

\definecolor{pink0} {HTML} {FCE4EC}
\definecolor{pink1} {HTML} {F8BBD0}
\definecolor{pink2} {HTML} {F48FB1}
\definecolor{pink3} {HTML} {F06292}
\definecolor{pink4} {HTML} {EC407A}
\definecolor{pink5} {HTML} {FF80AB}

\definecolor{brown0} {HTML} {D7CCC8}
\definecolor{brown1} {HTML} {BCAAA4}
\definecolor{brown2} {HTML} {A1887F}
\definecolor{brown3} {HTML} {8D6E63}
\definecolor{brown4} {HTML} {795548}
\definecolor{brown5} {HTML} {6D4C41}
\definecolor{brown6} {HTML} {5D4037}

\definecolor{yellow0} {HTML} {CDDC39}
\definecolor{yellow1} {HTML} {9E9D24}
\definecolor{yellow3} {HTML} {FFBD2A}
\definecolor{yellow4} {HTML} {FFB000}
\definecolor{yellow5} {HTML} {FFD600}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:
